Learning to Cluster under Domain Shift

While unsupervised domain adaptation methods based on deep architectures have achieved remarkable success in many computer vision tasks, they rely on a strong assumption, i.e. labeled source data must be available. In this work we overcome this assumption and we address the problem of transferring knowledge from a source to a target domain when both source and target data have no annotations. Inspired by recent works on deep clustering, our approach leverages information from data gathered from multiple source domains to build a domain-agnostic clustering model which is then refined at inference time when target data become available. Specifically, at training time we propose to optimize a novel information-theoretic loss which, coupled with domain-alignment layers, ensures that our model learns to correctly discover semantic labels while discarding domain-specific features. Importantly, our architecture design ensures that at inference time the resulting source model can be effectively adapted to the target domain without having access to source data, thanks to feature alignment and self-supervision. We evaluate the proposed approach in a variety of settings, considering several domain adaptation benchmarks and we show that our method is able to automatically discover relevant semantic information even in presence of few target samples and yields state-of-the-art results on multiple domain adaptation benchmarks.

==> egbib.bak.tex <==

@misc{Authors14,
 author = {Authors},
 title = {The frobnicatable foo filter},
 note = {{BMVC14} submission ID 324. Supplied as additional material {\tt bmvc14.pdf}},
 year = 2014
}

@misc{Authors14b,
 author = {Authors},
 title = {Frobnication tutorial},
 note = {Supplied as additional material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {A. Alpher},
title = {Frobnication},
journal = {Journal of Foo},
volume = 12,
number = 1,
pages = {234--778},
year = 2002
}

@article{Alpher03,
author = {A. Alpher and J.~P.~N. Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13,
number = 1,
pages = {234--778},
year = 2003
}

@article{Alpher04,
author = {A. Alpher and J.~P.~N. Fotheringham-Smythe and G. Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14,
number = 1,
pages = {234--778},
year = 2004
}

@article{carlucci2018agnostic,
  title={Agnostic Domain Generalization},
  author={Carlucci, Fabio M and Russo, Paolo and Tommasi, Tatiana and Caputo, Barbara},
  journal={arXiv preprint arXiv:1808.01102},
  year={2018}
}

@article{morerio2017minimal,
  title={Minimal-entropy correlation alignment for unsupervised deep domain adaptation},
  author={Morerio, Pietro and Cavazza, Jacopo and Murino, Vittorio},
  journal={ICLR},
  year={2018}
}

@inproceedings{carlucci2019domain,
  title={Domain Generalization by Solving Jigsaw Puzzles},
  author={Carlucci, Fabio M and D'Innocente, Antonio and Bucci, Silvia and Caputo, Barbara and Tommasi, Tatiana},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2229--2238},
  year={2019}
}

@inproceedings{roy2019unsupervised,
  title={Unsupervised domain adaptation using feature-whitening and consensus loss},
  author={Roy, Subhankar and Siarohin, Aliaksandr and Sangineto, Enver and Bulo, Samuel Rota and Sebe, Nicu and Ricci, Elisa},
  booktitle={CVPR},
  year={2019}
}


@inproceedings{LOAD_ICRA,
  author    = {Gabriele Angeletti and
               Barbara Caputo and
               Tatiana Tommasi},
  title     = {Adaptive Deep Learning through Visual Domain Localization},
  booktitle   = {ICRA},
  year      = {2018}
}

@inproceedings{li2017deeper,
  title={Deeper, broader and artier domain generalization},
  author={Li, Da and Yang, Yongxin and Song, Yi-Zhe and Hospedales, Timothy M},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={5542--5550},
  year={2017}
}

@inproceedings{xu2018deep,
  author    = {Ruijia Xu and
               Ziliang Chen and
               Wangmeng Zuo and
               Junjie Yan and
               Liang Lin},
  title     = {Deep Cocktail Network: Multi-source Unsupervised Domain Adaptation
               with Category Shift},
  booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year      = {2018}
}

@inproceedings{MDAN_ICLRW18,
  author    = {Han Zhao and
               Shanghang Zhang and
               Guanhang Wu and
               Jo{\~{a}}o P. Costeira and
               Jos{\'{e}} M. F. Moura and
               Geoffrey J. Gordon},
  title     = {Multiple Source Domain Adaptation with Adversarial Learning},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Workshop Track Proceedings},
  year      = {2018},
  crossref  = {DBLP:conf/iclr/2018w},
  url       = {https://openreview.net/forum?id=BkzXYSkvz},
  timestamp = {Thu, 04 Apr 2019 13:20:09 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/0002ZWCMG18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@proceedings{DBLP:conf/iclr/2018w,
  title     = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Workshop Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2018},
  url       = {https://openreview.net/group?id=ICLR.cc/2018/Workshop},
  timestamp = {Thu, 04 Apr 2019 13:20:09 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/2018w},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{hoffman2017cycada,
  title={CyCADA: Cycle-Consistent Adversarial Domain Adaptation},
  author={Hoffman, Judy and Tzeng, Eric and Park, Taesung and Zhu, Jun-Yan and Isola, Phillip and Saenko, Kate and Efros, Alexei and Darrell, Trevor},
  booktitle={Proceedings of the 35th International Conference on Machine Learning},
  year={2018}
}

@inproceedings{lee2013pseudo,
  title={Pseudo-label: The simple and efficient semi-supervised learning method for deep neural networks},
  author={Lee, Dong-Hyun},
  booktitle={Workshop on Challenges in Representation Learning, International Conference on Machine Learning},
  volume={3},
  pages={2},
  year={2013}
}

@InProceedings{chatfield2014return,
  author       = "Chatfield, K. and Simonyan, K. and Vedaldi, A. and Zisserman, A.",
  title        = "Return of the Devil in the Details: Delving Deep into Convolutional Nets",
  booktitle    = "British Machine Vision Conference",
  year         = "2014",
}

@inproceedings{venkateswara2017deep,
  title={Deep hashing network for unsupervised domain adaptation},
  author={Venkateswara, Hemanth and Eusebio, Jose and Chakraborty, Shayok and Panchanathan, Sethuraman},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5018--5027},
  year={2017}
}

@techreport{zhu2005semi,
  title={Semi-supervised learning literature survey},
  author={Zhu, Xiaojin Jerry},
  year={2005},
  institution={University of Wisconsin-Madison Department of Computer Sciences}
}

@article{Taigman2016UnsupervisedCI,
  title={Unsupervised Cross-Domain Image Generation},
  author={Yaniv Taigman and Adam Polyak and Lior Wolf},
  journal={International Conference on Learning Representations (ICLR)},
  year={2017},
}

@inproceedings{Shrivastava:arXiv:16,
  title={Learning from simulated and unsupervised images through adversarial training},
  author={Shrivastava, Ashish and Pfister, Tomas and Tuzel, Oncel and Susskind, Joshua and Wang, Wenda and Webb, Russell},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2107--2116},
  year={2017}
}

@inproceedings{Goodfellow:GAN:NIPS2014,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle={Advances in neural information processing systems},
  pages={2672--2680},
  year={2014}
}

@inproceedings{Bousmalis:Google:CVPR17,
  title = {Unsupervised Pixel-level Domain Adaptation with GANs},
  author  = {Konstantinos Bousmalis and Nathan Silberman and David Dohan and Dumitru Erhan and Dilip Krishnan},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2017},
}

@inproceedings{ADDA,
  author    = {Eric Tzeng and
               Judy Hoffman and
               Kate Saenko and
               Trevor Darrell},
  title     = {Adversarial Discriminative Domain Adaptation},
  booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year      = {2017}
}
% LOAD_ICRA
%@inproceedings{angeletti18,
%  author    = {Gabriele Angeletti and
%               Barbara Caputo and
%               Tatiana Tommasi},
%  title     = {Adaptive Deep Learning through Visual Domain Localization},
%  booktitle   = {International Conference on Robotic Automation (ICRA)},
%  year      = {2018}
%}

@inproceedings{chu2013selective,
  title={Selective transfer machine for personalized facial action unit detection},
  author={Chu, Wen-Sheng and De la Torre, Fernando and Cohn, Jeffery F},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2013}
}

@inproceedings{huang2006correcting,
  title={Correcting sample selection bias by unlabeled data},
  author={Huang, Jiayuan and Gretton, Arthur and Borgwardt, Karsten M and Sch{\"o}lkopf, Bernhard and Smola, Alex J},
  booktitle={Advances in neural information processing systems},
  year={2006}
}

@inproceedings{yamada2012no,
  title={No bias left behind: Covariate shift adaptation for discriminative 3d pose estimation},
  author={Yamada, Makoto and Sigal, Leonid and Raptis, Michalis},
  booktitle={European Conference on Computer Vision},
  pages={674--687},
  year={2012},
  organization={Springer}
}

@inproceedings{zeng2014deep,
  title={Deep learning of scene-specific classifier for pedestrian detection},
  author={Zeng, Xingyu and Ouyang, Wanli and Wang, Meng and Wang, Xiaogang},
  booktitle={European Conference on Computer Vision},
  year={2014}
}

@inproceedings{gong2013connecting,
  title={Connecting the dots with landmarks: Discriminatively learning domain-invariant features for unsupervised domain adaptation},
  author={Gong, Boqing and Grauman, Kristen and Sha, Fei},
  booktitle={International Conference on Machine Learning},
  pages={222--230},
  year={2013}
}


@inproceedings{long2013transfer,
  title={Transfer sparse coding for robust image representation},
  author={Long, Mingsheng and Ding, Guiguang and Wang, Jianmin and Sun, Jiaguang and Guo, Yuchen and Yu, Philip S},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2013}
}

@article{tzeng2014deep,
  title={Deep domain confusion: Maximizing for domain invariance},
  author={Tzeng, Eric and Hoffman, Judy and Zhang, Ning and Saenko, Kate and Darrell, Trevor},
  journal={arXiv preprint arXiv:1412.3474},
  year={2014}
}

@inproceedings{tzeng2015simultaneous,
  title={Simultaneous deep transfer across domains and tasks},
  author={Tzeng, Eric and Hoffman, Judy and Darrell, Trevor and Saenko, Kate},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  year={2015}
}



@article{ganin2014unsupervised,
  title={Unsupervised domain adaptation by backpropagation},
  author={Ganin, Yaroslav and Lempitsky, Victor},
  journal={International Conference on Machine Learning},
  year={2015}
}

@article{long2016unsupervised,
  title={Unsupervised Domain Adaptation with Residual Transfer Networks},
  author={Long, Mingsheng and Wang, Jianmin and Jordan, Michael I},
  journal={Advances in neural information processing systems},
  year={2016}
}

@inproceedings{li2016revisiting,
  author    = {Yanghao Li and
               Naiyan Wang and
               Jianping Shi and
               Jiaying Liu and
               Xiaodi Hou},
  title     = {Revisiting Batch Normalization For Practical Domain Adaptation},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Workshop Track Proceedings},
  year      = {2017},
  crossref  = {DBLP:conf/iclr/2017w},
  url       = {https://openreview.net/forum?id=Hk6dkJQFx},
  timestamp = {Thu, 04 Apr 2019 13:20:08 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/LiWS0H17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/iclr/2017w,
  title     = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Workshop Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2017},
  url       = {https://openreview.net/group?id=ICLR.cc/2017/workshop},
  timestamp = {Thu, 04 Apr 2019 13:20:08 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/2017w},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@ARTICLE{oneill1978normal,
    author = {O'Neill, T.~J.},
    title = {Normal discrimination with unclassified observations},
    journal = {Jounral of the American Statistical Association},
    year = {1978},
    pages={821--826},
    volume={73},
    number={364}
}

@inproceedings{sun2016deep,
  title={Deep coral: Correlation alignment for deep domain adaptation},
  author={Sun, Baochen and Saenko, Kate},
  booktitle={European Conference on Computer Vision},
  pages={443--450},
  year={2016},
  organization={Springer}
}

@inproceedings{ioffe2015batch,
  title={Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift},
  author={Ioffe, Sergey and Szegedy, Christian},
  booktitle={International Conference on Machine Learning},
  pages={448--456},
  year={2015}
}

@inproceedings{donahue2014decaf,
  title={DeCAF: A Deep Convolutional Activation Feature for Generic Visual Recognition.},
  author={Donahue, Jeff and Jia, Yangqing and Vinyals, Oriol and Hoffman, Judy and Zhang, Ning and Tzeng, Eric and Darrell, Trevor},
  booktitle={International Conference on Machine Learning},
  year={2014}
}

@ARTICLE{ben2010atheory,
    author = {Ben-David, S. and Blitzer, J. and Crammer, K. and Kulesza, A. and Pereira, F. and Vaughan, J.~W.},
    title = {A theory of learning from different domains},
    journal = {Machine Learning Journal},
    year = {2010},
    pages={151--175},
    volume={79},
    number={1--2}
}


@inproceedings{ben2010impossibility,
  author = {Ben-David, Shai and Lu, Tyler and Luu, Teresa and Pál, Dávid},
  booktitle = {AISTATS},
  title = {Impossibility Theorems for Domain Adaptation.},
  year = 2010
}


@inproceedings{tommasi2016learning,
  author    = {Tatiana Tommasi and
               Martina Lanzi and
               Paolo Russo and
               Barbara Caputo},
  title     = {Learning the Roots of Visual Domain Shift},
  booktitle = {Computer Vision - {European Conference on Computer Vision} 2016 Workshops - Amsterdam, The Netherlands,
               October 8-10 and 15-16, 2016, Proceedings, Part {III}},
  pages     = {475--482},
  year      = {2016},
  crossref  = {DBLP:conf/eccv/2016w3},
  url       = {https://doi.org/10.1007/978-3-319-49409-8\_39},
  doi       = {10.1007/978-3-319-49409-8\_39},
  timestamp = {Sun, 02 Jun 2019 21:17:49 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/eccv/TommasiLRC16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/eccv/2016w3,
  editor    = {Gang Hua and
               Herv{\'{e}} J{\'{e}}gou},
  title     = {Computer Vision - {ECCV} 2016 Workshops - Amsterdam, The Netherlands,
               October 8-10 and 15-16, 2016, Proceedings, Part {III}},
  series    = {Lecture Notes in Computer Science},
  volume    = {9915},
  year      = {2016},
  url       = {https://doi.org/10.1007/978-3-319-49409-8},
  doi       = {10.1007/978-3-319-49409-8},
  isbn      = {978-3-319-49408-1},
  timestamp = {Sun, 02 Jun 2019 21:17:49 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/eccv/2016w3},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{tommasi2014testbed,
  title={A testbed for cross-dataset analysis},
  author={Tommasi, Tatiana and Tuytelaars, Tinne},
  booktitle={European Conference on Computer Vision},
  year={2014}
}

@inproceedings{sun2016return,
  title={Return of Frustratingly Easy Domain Adaptation},
  author={Sun, Baochen and Feng, Jiashi and Saenko, Kate},
  booktitle={AAAI},
  year={2016}
}

@inproceedings{gong2012geodesic,
  title={Geodesic flow kernel for unsupervised domain adaptation},
  author={Gong, Boqing and Shi, Yuan and Sha, Fei and Grauman, Kristen},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2012}
}

@inproceedings{fernando2013unsupervised,
  title={Unsupervised visual domain adaptation using subspace alignment},
  author={Fernando, Basura and Habrard, Amaury and Sebban, Marc and Tuytelaars, Tinne},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  year={2013}
}

@inproceedings{russo17sbadagan,
  title={From source to target and back: symmetric bi-directional adaptive GAN},
  author={Russo, Paolo and Carlucci, Fabio Maria and Tommasi, Tatiana and Caputo, Barbara},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2018}
}

@article{pan2011domain,
  title={Domain adaptation via transfer component analysis},
  author={Pan, Sinno Jialin and Tsang, Ivor W and Kwok, James T and Yang, Qiang},
  journal={IEEE Transactions on Neural Networks},
  volume={22},
  number={2},
  pages={199--210},
  year={2011}
}

@inproceedings{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={Advances in neural information processing systems},
  pages={1097--1105},
  year={2012}
}

@inproceedings{saenko2010adapting,
  title={Adapting visual category models to new domains},
  author={Saenko, Kate and Kulis, Brian and Fritz, Mario and Darrell, Trevor},
  booktitle={European Conference on Computer Vision},
  year={2010}
}

@article{griffin2007caltech,
  title={Caltech-256 object category dataset},
  author={Griffin, Gregory and Holub, Alex and Perona, Pietro},
  year={2007},
  publisher={Technical report, California Institute of Technology}
}

@inproceedings{szegedy2015going,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2015}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2009}
}

@inproceedings{grandvalet2004semisupervised,
  author    = {Grandvalet, Y. and
               Bengio, Y.},
  title     = {Semi-supervised Learning by Entropy Minimization},
  booktitle = {Advances in neural information processing systems},
  year      = {2004},
}

@article{maaten2008visualizing,
  title={Visualizing data using t-SNE},
  author={Maaten, Laurens van der and Hinton, Geoffrey},
  journal={Journal of Machine Learning Research},
  volume={9},
  number={Nov},
  pages={2579--2605},
  year={2008}
}

@inproceedings{jia2014caffe,
  title={Caffe: Convolutional architecture for fast feature embedding},
  author={Jia, Yangqing and Shelhamer, Evan and Donahue, Jeff and Karayev, Sergey and Long, Jonathan and Girshick, Ross and Guadarrama, Sergio and Darrell, Trevor},
  booktitle={Proceedings of the 22nd ACM international conference on Multimedia},
  pages={675--678},
  year={2014},
  organization={ACM}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@inproceedings{long2017deep,
  title={Deep transfer learning with joint adaptation networks},
  author={Long, Mingsheng and Zhu, Han and Wang, Jianmin and Jordan, Michael I},
  booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
  pages={2208--2217},
  year={2017},
  organization={JMLR. org}
}

@inproceedings{ghifary2016deep,
  title={Deep Reconstruction-Classification Networks for Unsupervised Domain Adaptation},
  author={Ghifary, Muhammad and Kleijn, W Bastiaan and Zhang, Mengjie and Balduzzi, David and Li, Wen},
  booktitle={European Conference on Computer Vision},
  year={2016}
}

@InProceedings{haeusser17,
  author = 	 "P. Haeusser and T. Frerix and A. Mordvintsev and D. Cremers",
  title = 	 "Associative Domain Adaptation",
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  year = 	 "2017"
}

@incollection{TRUDA-NIPS16_savarese,
title = {Learning Transferrable Representations for Unsupervised Domain Adaptation},
author = {Sener, Ozan and Song, Hyun Oh and Saxena, Ashutosh and Savarese, Silvio},
booktitle = {Advances in Neural Information Processing Systems},
year = {2016},
}

@inproceedings{sankaranarayanan2017generate,
  title={Generate To Adapt: Aligning Domains using Generative Adversarial Networks},
  author={Sankaranarayanan, Swami and Balaji, Yogesh and Castillo, Carlos D and Chellappa, Rama},
booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
year={2018},
}

@inproceedings{bousmalis2016domain,
  title={Domain separation networks},
  author={Bousmalis, Konstantinos and Trigeorgis, George and Silberman, Nathan and Krishnan, Dilip and Erhan, Dumitru},
  booktitle={Advances in neural information processing systems},
  year={2016}
}

@inproceedings{yosinski2014transferable,
  title={How transferable are features in deep neural networks?},
  author={Yosinski, Jason and Clune, Jeff and Bengio, Yoshua and Lipson, Hod},
  booktitle={Advances in neural information processing systems},
  year={2014}
}

@inproceedings{aljundi2016lightweight,
  author    = {Rahaf Aljundi and
               Tinne Tuytelaars},
  title     = {Lightweight Unsupervised Domain Adaptation by Convolutional Filter
               Reconstruction},
  booktitle = {Computer Vision - {European Conference on Computer Vision} 2016 Workshop - Amsterdam, The Netherlands,
               October 8-10 and 15-16, 2016, Proceedings, Part {III}},
  pages     = {508--515},
  year      = {2016},
  crossref  = {DBLP:conf/eccv/2016w3},
  url       = {https://doi.org/10.1007/978-3-319-49409-8\_43},
  doi       = {10.1007/978-3-319-49409-8\_43},
  timestamp = {Sun, 02 Jun 2019 21:17:49 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/eccv/AljundiT16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{ganin2016domain,
  title={Domain-adversarial training of neural networks},
  author={Ganin, Yaroslav and Ustinova, Evgeniya and Ajakan, Hana and Germain, Pascal and Larochelle, Hugo and Laviolette, Fran{\c{c}}ois and Marchand, Mario and Lempitsky, Victor},
  journal={Journal of Machine Learning Research},
  volume={17},
  number={59},
  pages={1--35},
  year={2016}
}

@inproceedings{saito2017asymmetric,
  title={Asymmetric tri-training for unsupervised domain adaptation},
  author={Saito, Kuniaki and Ushiku, Yoshitaka and Harada, Tatsuya},
  booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
  pages={2988--2997},
  year={2017},
  organization={JMLR. org}
}

@inproceedings{netzer2011reading,
  title={Reading digits in natural images with unsupervised feature learning},
  author={Netzer, Yuval and Wang, Tao and Coates, Adam and Bissacco, Alessandro and Wu, Bo and Ng, Andrew Y},
  booktitle={Advances in neural information processing systems workshop on deep learning and unsupervised feature learning},
  pages={5},
  year={2011}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={IEEE}
}

@inproceedings{carlucci2017just,
  title={Just DIAL: DomaIn Alignment Layers for Unsupervised Domain Adaptation},
  author={Carlucci, Fabio Maria and Porzi, Lorenzo and Caputo, Barbara and Ricci, Elisa and Bul{\`o}, Samuel Rota},
  booktitle={ICIAP},
  year={2017}
}

@inproceedings{zen2014unsupervised,
  title={Unsupervised domain adaptation for personalized facial emotion recognition},
  author={Zen, Gloria and Sangineto, Enver and Ricci, Elisa and Sebe, Nicu},
  booktitle={ICMI},
  year={2014}
}

@inproceedings{costante2013transfer,
  title={A transfer learning approach for multi-cue semantic place recognition},
  author={Costante, Gabriele and Ciarfuglia, Thomas A and Valigi, Paolo and Ricci, Elisa},
  booktitle={IROS},
  year={2013}
}

@article{rozantsev2018beyond,
  title={Beyond sharing weights for deep domain adaptation},
  author={Rozantsev, Artem and Salzmann, Mathieu and Fua, Pascal},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={41},
  number={4},
  pages={801--814},
  year={2018},
  publisher={IEEE}
}

@inproceedings{ren2016normalizing,
  author    = {Mengye Ren and
               Renjie Liao and
               Raquel Urtasun and
               Fabian H. Sinz and
               Richard S. Zemel},
  title     = {Normalizing the Normalizers: Comparing and Extending Network Normalization
               Schemes},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  year      = {2017},
  crossref  = {DBLP:conf/iclr/2017},
  url       = {https://openreview.net/forum?id=rk5upnsxe},
  timestamp = {Thu, 04 Apr 2019 13:20:08 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/RenLUSZ17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@proceedings{DBLP:conf/iclr/2017,
  title     = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2017},
  url       = {https://openreview.net/group?id=ICLR.cc/2017/conference},
  timestamp = {Thu, 04 Apr 2019 13:20:07 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/2017},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{mancini2018boosting,
  title={Boosting domain adaptation by discovering latent domains},
  author={Mancini, Massimiliano and Porzi, Lorenzo and Rota Bul{\`o}, Samuel and Caputo, Barbara and Ricci, Elisa},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3771--3780},
  year={2018}
}

@article{mancini2018kitting,
  title={Kitting in the Wild through Online Domain Adaptation},
  author={Mancini, Massimiliano and Karaoguz, Hakan and Ricci, Elisa and Jensfelt, Patric and Caputo, Barbara},
  journal={IROS},
  year={2018}
}

@inproceedings{carlucci2017autodial,
  title={AutoDIAL: Automatic Domain Alignment Layers.},
  author={Carlucci, Fabio Maria and Porzi, Lorenzo and Caputo, Barbara and Ricci, Elisa and Bul{\`o}, Samuel Rota},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={5077--5085},
  year={2017}
}

@inproceedings{gopalan2011domain,
  title={Domain adaptation for object recognition: An unsupervised approach},
  author={Gopalan, Raghuraman and Li, Ruonan and Chellappa, Rama},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  year={2011}
}

@article{xie2015learning,
  title={Learning sparse frame models for natural image patterns},
  author={Xie, Jianwen and Hu, Wenze and Zhu, Song-Chun and Wu, Ying Nian},
  journal={IJCV},
  volume={114},
  number={2-3},
  pages={91--112},
  year={2015},
  publisher={Springer}
}

@inproceedings{lucic2018gans,
  title={Are gans created equal? a large-scale study},
  author={Lucic, Mario and Kurach, Karol and Michalski, Marcin and Gelly, Sylvain and Bousquet, Olivier},
  booktitle={Advances in neural information processing systems},
  pages={700--709},
  year={2018}
}

@article{wang2019generative,
  title={Generative Adversarial Networks: A Survey and Taxonomy},
  author={Wang, Zhengwei and She, Qi and Ward, Tomas E},
  journal={arXiv preprint arXiv:1906.01529},
  year={2019}
}

@book{csurka2017domain,
  title={Domain adaptation in computer vision applications},
  author={Csurka, Gabriela},
  volume={2},
  year={2017},
  publisher={Springer}
}

@inproceedings{DBLP:conf/iclr/BrockDS19,
  author    = {Andrew Brock and
               Jeff Donahue and
               Karen Simonyan},
  title     = {Large Scale {GAN} Training for High Fidelity Natural Image Synthesis},
  booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
               New Orleans, LA, USA, May 6-9, 2019},
  year      = {2019},
  crossref  = {DBLP:conf/iclr/2019},
  url       = {https://openreview.net/forum?id=B1xsqj09Fm},
  timestamp = {Thu, 25 Jul 2019 13:03:18 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/BrockDS19},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@proceedings{DBLP:conf/iclr/2019,
  title     = {7th International Conference on Learning Representations, {ICLR} 2019,
               New Orleans, LA, USA, May 6-9, 2019},
  publisher = {OpenReview.net},
  year      = {2019},
  url       = {https://openreview.net/group?id=ICLR.cc/2019/Conference},
  timestamp = {Thu, 25 Jul 2019 13:03:15 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/2019},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{karras2019style,
  title={A style-based generator architecture for generative adversarial networks},
  author={Karras, Tero and Laine, Samuli and Aila, Timo},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={4401--4410},
  year={2019}
}

@article{yoshida2017spectral,
  title={Spectral norm regularization for improving the generalizability of deep learning},
  author={Yoshida, Yuichi and Miyato, Takeru},
  journal={arXiv preprint arXiv:1705.10941},
  year={2017}
}

@article{DBLP:journals/corr/abs-1807-05520,
  author    = {Mathilde Caron and
               Piotr Bojanowski and
               Armand Joulin and
               Matthijs Douze},
  title     = {Deep Clustering for Unsupervised Learning of Visual Features},
  journal   = {CoRR},
  volume    = {abs/1807.05520},
  year      = {2018},
  url       = {http://arxiv.org/abs/1807.05520},
  archivePrefix = {arXiv},
  eprint    = {1807.05520},
  timestamp = {Mon, 13 Aug 2018 16:46:44 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1807-05520.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1807-06653,
  author    = {Xu Ji and
               Jo{\~{a}}o F. Henriques and
               Andrea Vedaldi},
  title     = {Invariant Information Distillation for Unsupervised Image Segmentation
               and Clustering},
  journal   = {CoRR},
  volume    = {abs/1807.06653},
  year      = {2018},
  url       = {http://arxiv.org/abs/1807.06653},
  archivePrefix = {arXiv},
  eprint    = {1807.06653},
  timestamp = {Mon, 13 Aug 2018 16:48:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1807-06653.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@book{goodfellow2016deep,
title={Deep learning},
author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron and Bengio, Yoshua},
volume={1},
year={2016},
publisher={MIT Press}
}

@inproceedings{long2015learning,
  title={Learning transferable features with deep adaptation networks},
  author={Long, Mingsheng and Wang, Jianmin},
  booktitle={ICML},
  year={2015}
}

%long2017deep
%@inproceedings{long2016deep,
%  title={Deep transfer learning with joint adaptation networks},
%  author={Long, Mingsheng and Zhu, Han and Wang, Jianmin and Jordan, Michael I},
%  booktitle={ICML},
%  year={2017}
%}




}

@inproceedings{peng2018synthetic,
  title={Synthetic to real adaptation with generative correlation alignment networks},
  author={Peng, Xingchao and Saenko, Kate},
  booktitle={WACV},
  year={2018}
}

%ADDA
%@inproceedings{tzeng2017adversarial,
%  title={Adversarial discriminative domain adaptation},
%  author={Tzeng, Eric and Hoffman, Judy and Saenko, Kate and Darrell, Trevor},
%  booktitle={CVPR},
%  year={2017}
%}
%Goodfellow:GAN:NIPS2014
%@inproceedings{goodfellow2014generative,
%  title={Generative adversarial nets},
%  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
%  booktitle={NIPS},
%  year={2014}
%}


@inproceedings{liu2016coupled,
  title={Coupled generative adversarial networks},
  author={Liu, Ming-Yu and Tuzel, Oncel},
  booktitle={NIPS},
  year={2016}
}

@inproceedings{sankaranarayanan2018generate,
  title={Generate to adapt: Aligning domains using generative adversarial networks},
  author={Sankaranarayanan, Swami and Balaji, Yogesh and Castillo, Carlos D and Chellappa, Rama},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{yao2010boosting,
  title={Boosting for transfer learning with multiple sources},
  author={Yao, Yi and Doretto, Gianfranco},
  booktitle={CVPR},
  year={2010}
}



@article{peng2018moment,
  title={Moment Matching for Multi-Source Domain Adaptation},
  author={Peng, Xingchao and Bai, Qinxun and Xia, Xide and Huang, Zijun and Saenko, Kate and Wang, Bo},
  journal={ICCV},
  year={2019}
}

@inproceedings{isola2017image,
  title={Image-to-image translation with conditional adversarial networks},
  author={Isola, Phillip and Zhu, Jun-Yan and Zhou, Tinghui and Efros, Alexei A},
  booktitle={CVPR},
  year={2017}
}

@inproceedings{zhu2017unpaired,
  title={Unpaired image-to-image translation using cycle-consistent adversarial networks},
  author={Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A},
  booktitle={CVPR},
  year={2017}
}

@inproceedings{choi2018stargan,
  title={Stargan: Unified generative adversarial networks for multi-domain image-to-image translation},
  author={Choi, Yunjey and Choi, Minje and Kim, Munyoung and Ha, Jung-Woo and Kim, Sunghun and Choo, Jaegul},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{murez2018image,
  title={Image to image translation for domain adaptation},
  author={Murez, Zak and Kolouri, Soheil and Kriegman, David and Ramamoorthi, Ravi and Kim, Kyungnam},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{perez2018film,
  title={Film: Visual reasoning with a general conditioning layer},
  author={Perez, Ethan and Strub, Florian and De Vries, Harm and Dumoulin, Vincent and Courville, Aaron},
  booktitle={AAAI},
  year={2018}
}

@inproceedings{huang2018multimodal,
  title={Multimodal unsupervised image-to-image translation},
  author={Huang, Xun and Liu, Ming-Yu and Belongie, Serge and Kautz, Jan},
  booktitle={ECCV},
  year={2018}
}

@inproceedings{anoosheh2018combogan,
  title={Combogan: Unrestrained scalability for image domain translation},
  author={Anoosheh, Asha and Agustsson, Eirikur and Timofte, Radu and Van Gool, Luc},
  booktitle={CVPR},
  year={2018}
}

%sun2016return
%@inproceedings{sun2016return,
%  title={Return of Frustratingly Easy Domain Adaptation},
%  author={Sun, Baochen and Feng, Jiashi and Saenko, Kate},
%  booktitle={AAAI},
%  year={2016}
%}


@ARTICLE{mancini2018robust,
author={M. Mancini and S. Rota Bul{\`o} and B. Caputo and E. Ricci},
journal={IEEE Robotics and Automation Letters},
title={Robust Place Categorization With Deep Domain Generalization},
year={2018},
volume={3},
number={3},
pages={2093-2100},
ISSN={},
month={July},}


%sun2016return
%@inproceedings{Sun:CORAL:AAAI16,
%  author={Baochen Sun and Jiashi Feng and Kate Saenko},
%  title={Return of Frustratingly Easy Domain Adaptation},
%  booktitle={AAAI},
%  year={2016}
%}

@inproceedings{WenLi:ECCV2016,
author="Ghifary, Muhammad
and Kleijn, W. Bastiaan
and Zhang, Mengjie
and Balduzzi, David
and Li, Wen",
booktitle = "ECCV",
title="Deep Reconstruction-Classification Networks for Unsupervised Domain Adaptation",
year="2016"
}

@incollection{TRUDA-NIPS16_savarese,
title = {Learning Transferrable Representations for Unsupervised Domain Adaptation},
author = {Sener, Ozan and Song, Hyun Oh and Saxena, Ashutosh and Savarese, Silvio},
booktitle = {NIPS},
year = {2016},
}

@InProceedings{haeusser17,
  author = 	 "P. Haeusser and T. Frerix and A. Mordvintsev and D. Cremers",
  title = 	 "Associative Domain Adaptation",
  booktitle={ICCV},
  year = 	 "2017"
}

@inproceedings{sankaranarayanan2017generate,
  title={Generate To Adapt: Aligning Domains using Generative Adversarial Networks},
  author={Sankaranarayanan, Swami and Balaji, Yogesh and Castillo, Carlos D and Chellappa, Rama},
booktitle={CVPR},
year={2018},
}
%ADDA
%@inproceedings{Hoffman:Adda:CVPR17,
%author={Eric Tzeng and Judy Hoffman and Trevor Darrell and Kate Saenko},
%title={Adversarial Discriminative Domain Adaptation},
%booktitle={CVPR},
%year={2017},
%}

%@inproceedings{LOAD_ICRA,
%  author    = {Gabriele Angeletti and
%               Barbara Caputo and
%               Tatiana Tommasi},
%  title     = {Adaptive Deep Learning through Visual Domain Localization},
%  booktitle   = {ICRA},
%  year      = {2018}
%}

%Bousmalis:Google:CVPR17
%@inproceedings{Bousmalis:Google:CVPR17,
%title = {Unsupervised Pixel-level Domain Adaptation with GANs},
%author  = {Konstantinos Bousmalis and Nathan Silberman and David Dohan and Dumitru %Erhan and Dilip Krishnan},
%booktitle={CVPR},
%year={2017},
%}
%Goodfellow:GAN:NIPS2014
%@incollection{Goodfellow:GAN:NIPS2014,
%title = {Generative Adversarial Nets},
%author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
%booktitle = {NIPS},
%year = {2014}
%}

%Shrivastava:arXiv:16
%@inproceedings{appleGAN,
%  title={Learning from Simulated and Unsupervised Images through Adversarial Training},
%  author={Ashish Shrivastava and Tomas Pfister and Oncel Tuzel and Joshua Susskind and Wenda Wang and Russell Webb},
%  booktitle={CVPR},
%  year={2017},
%}

@inproceedings{MLDG_AAA18,
  author    = {Da Li and
               Yongxin Yang and
               Yi{-}Zhe Song and
               Timothy M. Hospedales},
  title     = {Learning to Generalize: Meta-Learning for Domain Generalization},
  booktitle = {Conference of the Association for the Advancement of Artificial Intelligence (AAAI)},
  year      = {2018}
}

% MULTISOURCE PRACTICE %%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Crammer_JMLR08,
 author = {Crammer, Koby and Kearns, Michael and Wortman, Jennifer},
 title = {Learning from Multiple Sources},
 journal = {JMLR},
 year = {2008}
} 


%@inproceedings{MDAN_ICLRW18,
%title={Multiple Source Domain Adaptation with Adversarial Learning},
%author={Han Zhao and Shanghang Zhang and Guanhang Wu and Jo\~{a}o  P. Costeira and Jos\'{e} M. F.  Moura and Geoffrey J. Gordon},
%booktitle = {ICLR-WS},
%year={2018}
%}


@inproceedings{LongZ0J17,
  author    = {Mingsheng Long and
               Han Zhu and
               Jianmin Wang and
               Michael I. Jordan},
  title     = {Deep Transfer Learning with Joint Adaptation Networks},
  booktitle = {ICML},
  year      = {2017}
}



@inproceedings{hoffman2012discovering,
  title={Discovering latent domains for multisource domain adaptation},
  author={Hoffman, Judy and Kulis, Brian and Darrell, Trevor and Saenko, Kate},
  booktitle={ECCV},
  year={2012}
}
@book{friedman2001elements,
  title={The elements of statistical learning},
  author={Friedman, Jerome and Hastie, Trevor and Tibshirani, Robert},
  volume={1},
  year={2001},
  publisher={Springer series in statistics New York}
}

@inproceedings{bousmalis2016unsupervised,
  title={Unsupervised pixel-level domain adaptation with generative adversarial networks},
  author={Bousmalis, Konstantinos and Silberman, Nathan and Dohan, David and Erhan, Dumitru and Krishnan, Dilip},
   booktitle={CVPR},
  year={2017}
}
@article{xie2015learning,
  title={Learning sparse frame models for natural image patterns},
  author={Xie, Jianwen and Hu, Wenze and Zhu, Song-Chun and Wu, Ying Nian},
  journal={IJCV},
  volume={114},
  number={2-3},
  pages={91--112},
  year={2015},
  publisher={Springer}
}
@inproceedings{gopalan2011domain,
  title={Domain adaptation for object recognition: An unsupervised approach},
  author={Gopalan, Raghuraman and Li, Ruonan and Chellappa, Rama},
  booktitle={ICCV},
  year={2011}
}

@inproceedings{netzer2011reading,
  title={Reading digits in natural images with unsupervised feature learning},
  author={Netzer, Yuval and Wang, Tao and Coates, Adam and Bissacco, Alessandro and Wu, Bo and Ng, Andrew Y},
  booktitle={NIPS-WS},
  year={2011}
}


@inproceedings{gong2013reshaping,
  title={Reshaping visual datasets for domain adaptation},
  author={Gong, Boqing and Grauman, Kristen and Sha, Fei},
  booktitle={NIPS},
  year={2013}
}
@article{nguyen2015dash,
  title={DASH-N: Joint hierarchical domain adaptation and feature learning},
  author={Nguyen, Hien V and Ho, Huy Tho and Patel, Vishal M and Chellappa, Rama},
  journal={IEEE T-IP},
  volume={24},
  number={12},
  pages={5479--5491},
  year={2015},
  publisher={IEEE}
}
@article{gopalan2014unsupervised,
  title={Unsupervised adaptation across domain shifts by generating intermediate data representations},
  author={Gopalan, Raghuraman and Li, Ruonan and Chellappa, Rama},
  journal={IEEE T-PAMI},
  volume={36},
  number={11},
  pages={2288--2302},
  year={2014},
  publisher={IEEE}
}

@inproceedings{jhuo2012robust,
  title={Robust visual domain adaptation with low-rank reconstruction},
  author={Jhuo, I-Hong and Liu, Dong and Lee, DT and Chang, Shih-Fu},
  booktitle={CVPR},
  year={2012}
}


@article{lin2017cross,
  title={Cross-Domain Recognition by Identifying Joint Subspaces of Source Domain and Target Domain},
  author={Lin, Yuewei and Chen, Jing and Cao, Yu and Zhou, Youjie and Zhang, Lingfeng and Tang, Yuan Yan and Wang, Song},
  journal={IEEE Transactions on Cybernetics},
  volume={47},
  number={4},
  pages={1090--1101},
  year={2017},
  publisher={IEEE}
}

@article{gopalan2017image,
  title={Image Clustering Under Domain Shift},
  author={Gopalan, Raghuraman},
  year={2017},
  publisher={IEEE}
}


@inproceedings{shekhar2013generalized,
  title={Generalized domain-adaptive dictionaries},
  author={Shekhar, Sumit and Patel, Vishal M and Nguyen, Hien V and Chellappa, Rama},
  booktitle={CVPR},
  year={2013}
}
%Shrivastava:arXiv:16
%@inproceedings{shrivastava2017learning,
%  title={Learning From Simulated and Unsupervised Images Through Adversarial %Training},
%  author={Shrivastava, Ashish and Pfister, Tomas and Tuzel, Oncel and Susskind, Joshua and Wang, Wenda and Webb, Russell},
%  booktitle={CVPR},
%  year={2017}
%}


@article{li2017domain,
  title={Domain generalization and adaptation using low rank exemplar svms},
  author={Li, Wen and Xu, Zheng and Xu, Dong and Dai, Dengxin and Van Gool, Luc},
  journal={IEEE T-PAMI},
  year={2017},
  publisher={IEEE}
}


@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={IJCV},
  year={2015},
  publisher={Springer}
}
@article{arbelaez2011contour,
  title={Contour detection and hierarchical image segmentation},
  author={Arbelaez, Pablo and Maire, Michael and Fowlkes, Charless and Malik, Jitendra},
  journal={IEEE T-PAMI},
  volume={33},
  number={5},
  pages={898--916},
  year={2011},
  publisher={IEEE}
}
@article{srivastava2014dropout,
  title={Dropout: a simple way to prevent neural networks from overfitting.},
  author={Srivastava, Nitish and Hinton, Geoffrey E and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
  journal={JMLR},
  volume={15},
  number={1},
  pages={1929--1958},
  year={2014}
}
%gong2012geodesic
%@inproceedings{gong2012geodesic,
%  title={Geodesic flow kernel for unsupervised domain adaptation},
%  author={Gong, Boqing and Shi, Yuan and Sha, Fei and Grauman, Kristen},
%  booktitle={CVPR},
%  year={2012}
%}

@inproceedings{xiong2014latent,
  title={Latent Domains Modeling for Visual Domain Adaptation},
  author={Xiong, Caiming and McCloskey, Scott and Hsieh, Shao-Hang and Corso, Jason J},
  booktitle={AAAI},
  year={2014}
}



@article{pan2010survey,
  title={A survey on transfer learning},
  author={Pan, Sinno Jialin and Yang, Qiang},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={22},
  number={10},
  pages={1345--1359},
  year={2010}
}
%ben2010atheory
%@article{ben2010theory,
%  title={A theory of learning from different domains},
%  author={Ben-David, Shai and Blitzer, John and Crammer, Koby and Kulesza, Alex and Pereira, Fernando and Vaughan, Jennifer Wortman},
%  journal={Machine learning},
%  volume={79},
%  number={1},
%  pages={151--175},
%  year={2010}
%}

%chu2013selective
%@inproceedings{chu2013selective,
%  title={Selective transfer machine for personalized facial action unit detection},
%  author={Chu, Wen-Sheng and De la Torre, Fernando and Cohn, Jeffery F},
%  booktitle={CVPR},
%  year={2013}
%}

%@inproceedings{huang2006correcting,
%  title={Correcting sample selection bias by unlabeled data},
%  author={Huang, Jiayuan and Gretton, Arthur and Borgwardt, Karsten M and Sch{\"o}lkopf, Bernhard and Smola, Alex J},
%  booktitle={NIPS},
%  year={2006}
%}
%yamada2012no
%@inproceedings{yamada2012no,
%  title={No bias left behind: Covariate shift adaptation for discriminative 3D pose estimation},
%  author={Yamada, Makoto and Sigal, Leonid and Raptis, Michalis},
%  booktitle={ECCV},
%  year={2012}
%}

%zeng2014deep
%@inproceedings{zeng2014deep,
%  title={Deep learning of scene-specific classifier for pedestrian detection},
%  author={Zeng, Xingyu and Ouyang, Wanli and Wang, Meng and Wang, Xiaogang},
%  booktitle={ECCV},
%  year={2014}
%}
%gong2013connecting
%@inproceedings{gong2013connecting,
%  title={Connecting the Dots with Landmarks: Discriminatively Learning Domain-Invariant Features for Unsupervised Domain Adaptation.},
%  author={Gong, Boqing and Grauman, Kristen and Sha, Fei},
%  booktitle={ICML},
%  year={2013}
%}

%long2013transfer
%@inproceedings{long2013transfer,
%  title={Transfer sparse coding for robust image representation},
%  author={Long, Mingsheng and Ding, Guiguang and Wang, Jianmin and Sun, Jiaguang and Guo, Yuchen and Yu, Philip S},
%  booktitle={CVPR},
%  year={2013}
%}


%long2016unsupervised
%@article{long2016unsupervised,
%  title={Unsupervised Domain Adaptation with Residual Transfer Networks},
%  author={Long, Mingsheng and Wang, Jianmin and Jordan, Michael I},
%  journal={NIPS},
%  year={2016}
%}


%oneill1978normal
%@article{oneill1978normal,
%    author = {O'Neill, T.~J.},
%    title = {Normal discrimination with unclassified observations},
%    journal = {Journal of the American Statistical Association},
%    year = {1978},
%    pages={821--826},
%    volume={73},
%    number={364}
%}


%donahue2014decaf
%@inproceedings{donahue2014decaf,
%  title={DeCAF: A Deep Convolutional Activation Feature for Generic Visual Recognition.},
%  author={Donahue, Jeff and Jia, Yangqing and Vinyals, Oriol and Hoffman, Judy and Zhang, Ning and Tzeng, Eric and Darrell, Trevor},
%  booktitle={ICML},
%  year={2014}
%}

%ben2010atheory
%@ARTICLE{ben2010atheory,
%    author = {Ben-David, S. and Blitzer, J. and Crammer, K. and Kulesza, A. and Pereira, F. and Vaughan, J.~W.},
%    title = {A theory of learning from different domains},
%    journal = {Machine Learning Journal},
%    year = {2010},
%    pages={151--175},
%    volume={79},
%    number={1--2}
%}

%ben2010impossibility
%@inproceedings{ben2010impossibility,
%  author = {Ben-David, Shai and Lu, Tyler and Luu, Teresa and Pál, Dávid},
%  booktitle = {AISTATS},
%  title = {Impossibility Theorems for Domain Adaptation.},
%  year = 2010
%}

%tommasi2016learning
%@article{tommasi2016learning,
%  title={Learning the Roots of Visual Domain Shift},
%  author={Tommasi, Tatiana and Lanzi, Martina and Russo, Paolo and Caputo, Barbara},
%  journal={arXiv:1607.06144},
%  year={2016}
%}

%tommasi2014testbed
%@inproceedings{tommasi2014testbed,
%  title={A testbed for cross-dataset analysis},
%  author={Tommasi, Tatiana and Tuytelaars, Tinne},
%  booktitle={ECCV},
%  year={2014}
%}
%fernando2013unsupervised
%@inproceedings{fernando2013unsupervised,
%  title={Unsupervised visual domain adaptation using subspace alignment},
%  author={Fernando, Basura and Habrard, Amaury and Sebban, Marc and Tuytelaars, Tinne},
%  booktitle={ICCV},
%  year={2013}
%}

%he2016deep
%@article{he2015deep,
%  title={Deep residual learning for image recognition},
%  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
%  journal={arXiv:1512.03385},
%  year={2015}
%}

@inproceedings{ghifary2016deep,
  title={Deep Reconstruction-Classification Networks for Unsupervised Domain Adaptation},
  author={Ghifary, Muhammad and Kleijn, W Bastiaan and Zhang, Mengjie and Balduzzi, David and Li, Wen},
  booktitle={ECCV},
  year={2016}
}

@inproceedings{bousmalis2016domain,
  title={Domain separation networks},
  author={Bousmalis, Konstantinos and Trigeorgis, George and Silberman, Nathan and Krishnan, Dilip and Erhan, Dumitru},
  booktitle={NIPS},
  year={2016}
}

@inproceedings{yosinski2014transferable,
  title={How transferable are features in deep neural networks?},
  author={Yosinski, Jason and Clune, Jeff and Bengio, Yoshua and Lipson, Hod},
  booktitle={NIPS},
  year={2014}
}

@inproceedings{aljundi2016lightweight,
  title={Lightweight Unsupervised Domain Adaptation by Convolutional Filter Reconstruction},
  author={Aljundi, Rahaf and Tuytelaars, Tinne},
  booktitle={ECCV TASK-CV Workshops},
  year={2016}
}

@article{ganin2016domain,
  title={Domain-adversarial training of neural networks},
  author={Ganin, Yaroslav and Ustinova, Evgeniya and Ajakan, Hana and Germain, Pascal and Larochelle, Hugo and Laviolette, Fran{\c{c}}ois and Marchand, Mario and Lempitsky, Victor},
  journal={JMLR},
  year={2016}
}

@article{saito2017asymmetric,
  title={Asymmetric Tri-training for Unsupervised Domain Adaptation},
  author={Saito, Kuniaki and Ushiku, Yoshitaka and Harada, Tatsuya},
  journal={arXiv:1702.08400},
  year={2017}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  year={1998}
}




@inproceedings{yang2007adapting,
  title={Adapting SVM classifiers to data with shifted distributions},
  author={Yang, Jun and Yan, Rong and Hauptmann, Alexander G},
  booktitle={ICDM-WS 2007},
  year={2007}
}

@inproceedings{mansour2009domain,
  title={Domain adaptation with multiple sources},
  author={Mansour, Yishay and Mohri, Mehryar and Rostamizadeh, Afshin},
  booktitle={NIPS},
  year={2009}
}

@inproceedings{duan2009domain,
  title={Domain adaptation from multiple sources via auxiliary classifiers},
  author={Duan, Lixin and Tsang, Ivor W and Xu, Dong and Chua, Tat-Seng},
  booktitle={ICML},
  year={2009}
}

@inproceedings{sun2011two,
  title={A two-stage weighting framework for multi-source domain adaptation},
  author={Sun, Qian and Chattopadhyay, Rita and Panchanathan, Sethuraman and Ye, Jieping},
  booktitle={NIPS},
  year={2011}
}

@inproceedings{torralba2011unbiased,
  title={Unbiased look at dataset bias},
  author={Torralba, Antonio and Efros, Alexei A},
  booktitle={CVPR},
  year={2011}
}

@inproceedings{DBLP:journals/corr/DumoulinSK16,
  author    = {Vincent Dumoulin and
               Jonathon Shlens and
               Manjunath Kudlur},
  title     = {A Learned Representation For Artistic Style},
  booktitle   = {ICLR},
  year      = {2016},
}


@inproceedings{2018arXiv180600420S,
   author = {{Siarohin}, Aliaksandr and {Sangineto}, Enver and {Sebe}, Nicu},
    title = "{Whitening and Coloring batch transform for GANs}",
  booktitle = {ICLR},
     year = 2019,
}

@inproceedings{miyato2018cgans,
  title={cGANs with projection discriminator},
  author={Miyato, Takeru and Koyama, Masanori},
  booktitle={ICLR},
  year={2018}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv :1412.6980},
  year={2014}
}

@article{DBLP:journals/corr/UlyanovVL16,
  author    = {Dmitry Ulyanov and
               Andrea Vedaldi and
               Victor S. Lempitsky},
  title     = {Instance Normalization: The Missing Ingredient for Fast Stylization},
  journal   = {arXiv:1607.08022},
  year      = {2016},
}


@inproceedings{gatys2016image,
    author={Gatys, Leon A and Ecker, Alexander S and Bethge, Matthias},
    booktitle={CVPR},
    title={Image Style Transfer Using Convolutional Neural Networks},
    year={2016}
}

@inproceedings{jaderberg2015spatial,
  title={Spatial transformer networks},
  author={Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and others},
  booktitle={NIPS},
  year={2015}
}

@inproceedings{heusel2017gans,
  title={Gans trained by a two time-scale update rule converge to a local nash equilibrium},
  author={Heusel, Martin and Ramsauer, Hubert and Unterthiner, Thomas and Nessler, Bernhard and Hochreiter, Sepp},
  booktitle={NIPS},
  year={2017}
}

@article{yu2018multi,
  title={Multi-mapping image-to-image translation with central biasing normalization},
  author={Yu, Xiaoming and Ying, Zhenqiang and Li, Ge and Gao, Wen},
  journal={arXiv:1806.10050},
  year={2018}
}

@inproceedings{bousmalis2017unsupervised,
  title={Unsupervised pixel-level domain adaptation with generative adversarial networks},
  author={Bousmalis, Konstantinos and Silberman, Nathan and Dohan, David and Erhan, Dumitru and Krishnan, Dilip},
  booktitle={CVPR},
  year={2017}
}

%Taigman2016UnsupervisedCI
%@article{taigman2016unsupervised,
% title={Unsupervised cross-domain image generation},
%  author={Taigman, Yaniv and Polyak, Adam and Wolf, Lior},
%  journal={arXiv preprint arXiv:1611.02200},
%  year={2016}
%}

@inproceedings{liu2017unsupervised,
  title={Unsupervised image-to-image translation networks},
  author={Liu, Ming-Yu and Breuel, Thomas and Kautz, Jan},
  booktitle={NIPS},
  year={2017}
}

@inproceedings{larsson2016learning,
  title={Learning representations for automatic colorization},
  author={Larsson, Gustav and Maire, Michael and Shakhnarovich, Gregory},
  booktitle={European Conference on Computer Vision},
  year={2016}
}

@inproceedings{zhao2019geometry,
  title={Geometry-aware symmetric domain adaptation for monocular depth estimation},
  author={Zhao, Shanshan and Fu, Huan and Gong, Mingming and Tao, Dacheng},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2019}
}

@inproceedings{haeusser,
  title={Associative deep clustering:
Training a classification network with no labels},
  author={Haeusser, Philip and Plapp, Johannes and Golkov, Vladimir and Aljalbout, Elie and and Cremers, Daniel.},
  booktitle={German
Conference on Pattern Recognitionn},
  year={2018}
}

@inproceedings{liu2015deep,
  title={Deep learning face attributes in the wild},
  author={Liu, Ziwei and Luo, Ping and Wang, Xiaogang and Tang, Xiaoou},
  booktitle={ICCV},
  year={2015}
}

@inproceedings{li2019episodic,
  title={Episodic training for domain generalization},
  author={Li, Da and Zhang, Jianshu and Yang, Yongxin and Liu, Cong and Song, Yi-Zhe and Hospedales, Timothy M},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={1446--1455},
  year={2019}
}

%DBLP:journals/corr/abs-1903-07062
@inproceedings{mancini2019adagraph,
  title={Adagraph: Unifying predictive and continuous domain adaptation through graphs},
  author={Mancini, Massimiliano and Bulo, Samuel Rota and Caputo, Barbara and Ricci, Elisa},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6568--6577},
  year={2019}
}

@inproceedings{wang2017transitive,
  title={Transitive invariance for self-supervised visual representation learning},
  author={Wang, Xiaolong and He, Kaiming and Gupta, Abhinav},
  booktitle={Proceedings of the IEEE international conference on computer vision},
   year={2017}
}

@inproceedings{noroozi2016unsupervised,
  title={Unsupervised learning of visual representations by solving jigsaw puzzles},
  author={Noroozi, Mehdi and Favaro, Paolo},
  booktitle={European Conference on Computer Vision},
  pages={69--84},
  year={2016},
}

@article{siarohin2018whitening,
  title={Whitening and Coloring batch transform for GANs},
  author={Siarohin, Aliaksandr and Sangineto, Enver and Sebe, Nicu},
  journal={ICLR},
  year={2018}
}

@inproceedings{cho2019image,
  title={Image-to-image translation via group-wise deep whitening-and-coloring transformation},
  author={Cho, Wonwoong and Choi, Sungha and Park, David Keetae and Shin, Inkyu and Choo, Jaegul},
  booktitle={CVPR},
  year={2019}
}

@inproceedings{zhang2018unreasonable,
  title={The unreasonable effectiveness of deep features as a perceptual metric},
  author={Zhang, Richard and Isola, Phillip and Efros, Alexei A and Shechtman, Eli and Wang, Oliver},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{hung2019scops,
  title={SCOPS: Self-Supervised Co-Part Segmentation},
  author={Hung, Wei-Chih and Jampani, Varun and Liu, Sifei and Molchanov, Pavlo and Yang, Ming-Hsuan and Kautz, Jan},
  booktitle={CVPR},
  year={2019}
}

@inproceedings{dereniowski2003cholesky,
  title={Cholesky factorization of matrices in parallel and ranking of graphs},
  author={Dereniowski, Dariusz and Kubale, Marek},
  booktitle={International Conference on Parallel Processing and Applied Mathematics},
  year={2003},
}

@misc{sohn2020fixmatch,
    title={FixMatch: Simplifying Semi-Supervised Learning with Consistency and Confidence},
    author={Kihyuk Sohn and David Berthelot and Chun-Liang Li and Zizhao Zhang and Nicholas Carlini and Ekin D. Cubuk and Alex Kurakin and Han Zhang and Colin Raffel},
    year={2020},
    eprint={2001.07685},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}
